Revisiting Spectral Bundle Methods: Primal-dual (Sub)linear Convergence Rates

The spectral bundle method proposed by Helmberg and Rendl is well established for solving large-scale semidefinite programs (SDP) thanks to its low per iteration computational complexity and strong practical performance. In this paper, we revisit this classic method showing it achieves sublinear convergence rates in terms of both primal and dual SDPs under merely strong duality, complementing previous guarantees on primal-dual convergence. Moreover, we show the method speeds up to linear convergence if (1) structurally, the SDP admits strict complementarity, and (2) algorithmically, the bundle method captures the rank of the optimal solutions. Such complementary and low rank structure is prevalent in many modern and classical applications. The linear convergent result is established via an eigenvalue approximation lemma which might be of independent interest. Numerically, we confirm our theoretical findings that the spectral bundle method, for modern and classical applications, speeds up under these conditions. Finally, we show that the spectral bundle method combined with a recent matrix sketching technique is able to solve an SDP with billions of decision variables in a matter of minutes.

==> sketching.tex <==

\section{Storage reduction via matrix sketching and solving large scale problem} \label{sec: matrixSketching}
A particular bottleneck in solving large-scale problems is storing the primal matrix $X_t$. Here we show how to avoid storing this iterate by introducing the matrix sketching idea developed in \cite{tropp2017fixed,tropp2017practical,yurtsever2017sketchy} and demonstrate its usage for problems considered in Section \ref{sec: numerics}. Applying $(\rpast,\rcurrent)$-SpecBM with such a sketching procedure, we demonstrate this scalability improvement by solving a matrix completion SDP with approximately one billion decision variables (i.e., $(4\times 10^4)\times(4\times 10^4)$) in less than three minutes.

\subsection{The matrix sketching idea}
\newcontent{Let us introduce the matrix sketching idea introduced in \cite{tropp2017fixed,tropp2017practical,yurtsever2017sketchy}. Such procedure allows us to omit storing the aggregation $\bar{X}_{t+1}= \eta^\star_t \bar{X}_t +V_tQ_2\Lambda_2Q_2^\top V_t^\top$ and the primal iterate $X_{t} = \eta^\star_{t}\bar{X}_{t}+V_{t} S^\star_{t} V_{t}^\top$ using $\bigO(n^2)$ storage.
}

\newcontent{
We first draw a random matrix $\Psi \in \real^ {n \times R}$ with independent standard normal entries:
\begin{equation} \label{eq: randompsi}
\Psi \in \real^ {n \times R}\quad \text{with}\quad R= 3r+1,\quad\text{and}\quad \Psi_{ij} \overset{\text{iid}}{\sim} N(0,1).
\end{equation}
Here $r$ is chosen by the user. It either represents the estimate of the true rank of the primal solution or the user's computational budget in dealing with larges matrices. Next,
we form the sketches $\bar{Y}_t$ and $Y_t$ of $\bar{X}_t$ and $X_t$ respectively via 
\begin{equation}\label{eqn: onetimeSketch}
\bar{Y}_t = \bar{X}_t\Psi \in \real^{\dm \times R},\quad \text{and}\quad 
Y_t = X_t\Psi \in \real^{\dm \times R}.
\end{equation}
To avoid computing $\bar{Y}_t$ and $Y_t$ directly via the formulas \eqref{eqn: onetimeSketch}, we update them gradually using the updating formula of $X_t$ and $\bar{X}_t$ ($\bar{X}_{t+1} = \eta^\star_t \bar{X}_t +V_tQ_2\Lambda_2Q_2^\top V_t^\top$
and 
$X_{t} = \eta^\star_t\bar{X}_t+V_t S^\star_t V_t^\top$),
\begin{align}
\bar{Y}_{t+1} = V_tQ_2\Lambda_2Q_2^\top (V_t^\top\Psi)+ \eta_t^\star  \bar{Y}_t \in \real^{\dm \times R }, \label{eq:sketch-agg-update}\\
Y_{t+1} = V_{t+1}S^\star _{t+1}(V_{t+1}^\top\Psi)+ \eta_{t+1}^\star  \bar{Y}_{t+1} \in \real^{\dm \times R }. \label{eq:sketch-primal-update1}
\end{align}
We initialize $Y_0=\tilde{Y}_0 =0$. 
}
%This observation allows us to form the sketch $Y^C_t$ and $Y^R_t$ from the stream of updates. 
Finally, we reconstruct $X_t$ via 
\begin{align}\label{eqn: reconstructionsketch}
\hat{X}_t:= Y_t(\Psi^\top Y_t)^{\dagger}Y_t^\top.
\end{align}
Here $(\Psi^\top Y_t)^{\dagger}$ is the pseudo-inverse of $\Psi^\top Y_t$. Note that $\hat{X}_t$ is positive semidefinite since $X_t$ is and $\Psi^\top Y_t = \Psi^\top X_t\Psi_t$. A numerical stable implementation of \eqref{eqn: reconstructionsketch} can be found in \cite[Algorithm 3]{tropp2017fixed} and it outputs $(U_t,\Lambda_t)$ where $\hat{X}_t=U_t \Lambda_t U_t^\top$ with $U_t \in \real^{n\times R}$ with orthonromal columns and a nonnegative diagonal $\Lambda_t$. 
%(LD: I include one in the appendix \ref{sec: stable reconstruction}. Do we want to include it?)\todo{This stable construction seems nearly identical to the tropp2017 paper. Citing them should suffice.} 
Note that we store $\hat{X}_t$ via the factors $(U_t,\Lambda_t)$ rather than forming $\hat{X}_t$ explicitly, and their reconstruction only needs to be done whenever a primal matrix is needed instead of in every iteration.
From \cite[Theorem 4.1]{tropp2017fixed}, we have the following guarantee:
\begin{equation}\label{eq: sketchbound}
    \mathbb{E}_{\Psi}\|X_t - \hat{X}_t\|_*\leq \frac{4}{3}\|X_t -[X_t]_r\|_*,
\end{equation}
where $\|\cdot\|_*$ is the nuclear norm and $[\cdot]_r$ is the best rank $r$ approximation in terms of Frobenius norm. Hence, if $X_t$ is converging to a low rank matrix $\xsol$, then so long as $r\geq \rsol$, the approximation error $X_t-\hat{X}_t$ is small. 

%Specifically, the best rank $r$ approximation of a matrix $Z$ is $U\Sigma V^\top $,
%where $U$ and $V$ are right and left singular vectors corresponding to the $r$
%largest singular values of $Z$ and $\Sigma$ is a diagonal matrix with $r$ largest singular values of $Z$. 
%In actual implementation, one
%only needs the factors $(QU, \Sigma, V)$ defining the last iterate $\hat{X}_T$ instead of reconstructing $\hat{X}_t$ in every iteration. We refer the reader to \cite[Theorem 5.1]{tropp2017practical} for the theoretical guarantees on the reconstruction matrix $\hat{X}_t$.

\newcontent{Thus we can avoid \emph{forming new iterates} $\bar{X}_t$ and $X_t$, which occupies $\bigO(n^2)$ storage.
As discussed in the end of Section \ref{sec: ImportantsubproblemSolver}, we know that we can solve 
the subproblem \eqref{eq: subproblemAMSpectralbundleMethod} by storing $d_t = \Amap \bar{X}_t$, $c_t = \inprod{C}{\bar{X}_t}$, and $h_t=\tr(\bar{X}_t)$ rather than computing them directly from $\bar{X}_t$. Hence,
$(\rpast,\rcurrent)$-SpecBM combined with the matrix sketching idea described above, we only need a storage of size 
\begin{equation}\label{eq: storagesizeMsketching}
    \bigO(\underbrace{nr}_{\text{storing $\Psi$, $\bar{Y}_t$, and $Y_t$}} +\underbrace{m}_{\text{storing $d_t, \,c_t$, and $h_t$}}).
\end{equation}
The quantity $\bigO(nr + m)$ can be significantly smaller than $\bigO(n^2)$ for 
applications of SDP \eqref{p} when the rank estimate $r$ is small (constant or logarithmic with respect to $n$) and $m$ is on the order of $n$, see \cite{ding2019optimal} and \cite{yurtsever2017sketchy} for more discussions on the storage benefit.
}

%
%\newcontent{Another natural idea to store $X_t$ while avoiding $\bigO(n^2)$ storage is to store a factorization of it, e.g., eigenvalue decomposition. If the number of nonzero eigenvalues is small, then we can have much savings. However, as demonstrated in Appendix \ref{sec: plotsOfRank}, the rank of $X_t$ during the algorithmic process can be much larger than the rank of the solution $\rank(\xsol)$. Hence, storing $X_t$ in a factorization form during the initial and intermediate phase of the algorithm is not as beneficial as the matrix sketching procedure described above.
%\section{Plots of rank of $X_t$}\label{sec: plotsOfRank}
%
\subsection{Continuation of Matrix Completion and Max-Cut Experiments}
\newcontent{Continuing the experimental setup of Section~\ref{sec: numerics}, we demonstrate the usage of the matrix sketching procedure here.
First, in Figure \ref{fig: Xt rank}, we measure the numerical rank of $X_t$ (measured by the number of singular values larger than $10^{-2}$). 
We see that the intermediate rank of $X_t$ can be much larger than the primal optimal solution rank, $\rank(\xsol)$, even though in the end, its rank can be very close to or equal to $\rank(\xsol)$.
This is a particularly relevant observation in justifying the use of sketching procedures as only a low rank sketch of the primal solution matrix needs to be stored. While natural ideas such as storing $X_t$ via its factorization of it, e.g., eigenvalue decomposition, could still cause high storage due to intermediate high rank iterates.}
\begin{figure}[h]
	\begin{subfigure}[(a)]{.49\textwidth}
		\centering
		\includegraphics[width=1\linewidth, height= 0.25\textheight]{figures/MatrixCompletionXrank.png}
		\caption{Matrix Completion where $\text{rank}(X_\star)=3$}
		\label{fig:figure Matrix Completion Xt rank}
	\end{subfigure}%
	\hspace{5pt}
	\begin{subfigure}[(b)]{.49\textwidth}
		\centering
		\includegraphics[width=1\linewidth, height= 0.25\textheight]{figures/MaxCutPrimalRank.png}
		\caption{Max-cut where $\text{rank}(X_\star)=18$}
		\label{fig:figure Max-cut Xt rank}
	\end{subfigure}
	\caption{The evolution of the rank of the converging primal sequence $X_t$.}
	\label{fig: Xt rank}
\end{figure}
\begin{figure}[h]
	\begin{subfigure}[(a)]{.49\textwidth}
		\centering
		\includegraphics[width=1\linewidth, height= 0.25\textheight]{figures/sketchingIterateDiffMatrixCompletion.png}
		\caption{Matrix Completion where $\text{rank}(X_\star)=3$}
		\label{fig:figure Matrix Completion Xt rank}
	\end{subfigure}%
	\hspace{5pt}
	\begin{subfigure}[(b)]{.49\textwidth}
		\centering
		\includegraphics[width=1\linewidth, height= 0.25\textheight]{figures/maxcutsketching.png}
		\caption{Max-cut where $\text{rank}(X_\star)=18$}
		\label{fig:figure Max-cut Xt rank}
	\end{subfigure}
	\caption{The evolution of the difference  $\frac{\fronorm{X_t-\hat{X}_t}}{\fronorm{X_t}}$ between the sketching primal sequence $\hat{X}_t$ and the primal sequence $X_t$.}
	\label{fig: Primal Sketching}
\end{figure}

Next, we measure the relative difference between the reconstruction $\hat{X}_t$ and $X_t$. We set $R=10$ for the case of matrix completion and $R=60$ for the case of max-cut. Note that this is only for demonstration, in practice, one does not need to reconstruct $\hat{X}_t$ in every iteration but only reconstruct it whenever needed. As observed from Figure \ref{fig: Primal Sketching}, we see that even though in the beginning the difference $\frac{\fronorm{X_t-\hat{X}_t}}{\fronorm{X_t}}$ is large, in the end, the difference is negligible comparing to the primal optimality and feasibility of $X_t$.

\subsection{Large-scale Max Completion Experiments} Finally, we demonstrate that we are able to solve much larger problems using $(\rpast,\rcurrent)$-SpecBM with the matrix sketching procedure described above. We measure the running time via the wall-clock time, and the storage using the \texttt{peak memory} in Matlab \cite{MATLAB:R2021a} \texttt{profile} for 
$(\rpast,\rcurrent)$-SpecBM, which stores and forms $X_t,\bar{X}_t$ explicitly, and $(\rpast,\rcurrent)$-SpecBM with the matrix sketching (Sketching $(\rpast,\rcurrent)$-SpecBM). 

Because of the ease of computing the optimal solution and controlling its rank for the simulated matrix completion problem, we focus on this problem in this section. We follow the setting of matrix completion in Section \ref{sec: numerics} but vary the dimension of $X^\natural$ and the observation probability $p = \frac{80}{n}$. The resulting primal matrix size $n$ of the SDP is $n=5000$, $n=10^4$, $n = 2\times 10^4$, and $n= 4\times 10^4$. We set $\rpast = 0$ and $\rcurrent =4$ due to the good performance for the setting $n=2000$. We measure the performance of the two methods by the relative recovery error $\frac{\fronorm{\hat{X}-X^\natural}}{{\fronorm{X^\natural}}}$, where $\hat{X}$ is extracted from the left top $n\times n$ block of the final iterate $X_{100}$. The results are shown in Table \ref{tab: comparison}.
% \begin{table}[h]
% \begin{center}
% \begin{tabular}{||c c c c||} 
%  \hline 
%  $n$ & Time (s) & Storage (Kb) & Accuracy \\ [0.5ex] 
%  \hline\hline
%  $5000$ & 75.3764/33.6612 & 195316/48,832 & $2.8597\times 10^{-5}/2.9573\times 10^{-5}$\\ 
%  \hline
%  $10^4$ &   335.5/40.8492 & 781,256/196,333 & $5.3738\times 10^{-5}/1.004\times 10^{-4}$\\ 
%  \hline
%  $2\times 10^4$ & $\infty$/$61.0287$ & 3,123,621/781,324 & n.a./$3.2897\times 10^{-5}$ \\
%  \hline
%  $4\times 10^4$ & $\infty$/$140.6755$ & $\infty$/3,126,184 & n.a./$1.1777\times 10^{-4}$ \\
%  \hline
% \end{tabular}
% \end{center}
%     \caption{Comparison of $(0,4)$-SpecBM (left) and sketching $(0,4)$-SpecBM (right) for the matrix completion SDP. The symbol $\infty$ for time means the method does not finish within 3 hours. For storage, it means the method requires memory over 8GB.}
%     \label{tab: comparison}
% \end{table}
\begin{table}[h]
\begin{center}
\begin{tabular}{||c | c c c | c c c ||} 
 \hline 
 & \multicolumn{3}{c}{Without Sketching} & \multicolumn{3}{c}{With Sketching}\\
 \hline 
 $n$ & Time(s) & Storage (Kb) & Accuracy & Time(s) & Storage(Kb) & Accuracy \\ [0.5ex] 
 \hline\hline
 $5000$ & 75.38 & 195,316 & $2.86\times 10^{-5}$ & 33.66 & 48,832 & $2.96\times 10^{-5}$ \\ 
 \hline
 $10^4$ & 335.5 & 781,256 & $5.37\times 10^{-5}$ & 40.84 & 196,333 & $1.0\times 10^{-4}$\\ 
 \hline
 $2\times 10^4$ & $\infty$ & 3,123,621 & n.a. & $61.02$ & 781,324 & $3.29\times 10^{-5}$ \\
 \hline
 $4\times 10^4$ & $\infty$ & $\infty$ & n.a. & $140.67$ & 3,126,184 & $1.18\times 10^{-4}$\\
 \hline
\end{tabular}
\end{center}
    \caption{Comparison of $(0,4)$-SpecBM (left) and sketching $(0,4)$-SpecBM (right) for the matrix completion SDP. The symbol $\infty$ for time means the method does not finish within 3 hours. For storage, it means the method requires memory over 8GB.}
    \label{tab: comparison}
\end{table}
